CryptoNAS: Private Inference on a ReLU Budget

Machine learning as a service has given raise to privacy concerns surrounding clients' data and providers' models and has catalyzed research in private inference (PI): methods to process inferences without disclosing inputs. Recently, researchers have adapted cryptographic techniques to show PI is possible, however all solutions increase inference latency beyond practical limits. This paper makes the observation that existing models are ill-suited for PI and proposes a novel NAS method, named CryptoNAS, for finding and tailoring models to the needs of PI. The key insight is that in PI operator latency cost are non-linear operations (e.g., ReLU) dominate latency, while linear layers become effectively free. We develop the idea of a ReLU budget as a proxy for inference latency and use CryptoNAS to build models that maximize accuracy within a given budget. CryptoNAS improves accuracy by 3.4% and latency by 2.4x over the state-of-the-art.

==> tab_depth_vs_relubdg_comp.tex <==
%\begin{wraptable}{r}{0.6\textwidth}
\begin{table}[]
\caption{Accuracy of networks generated by \sys for different ReLU budgets.
\fixme{\sys scales all D(=3) networks to desired relu budgets (these are the networks produced at l:16 of Algo) and picks the best performing one as the final model for that budget. we pick the pareto points in this table and plot them in fig \ref{fig:acc_time}}}
\begin{tabular}{lcccc}\toprule
\multicolumn{1}{c}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Model \\ (Base-Budget)\end{tabular}}} & \multicolumn{2}{c}{CIFAR-10} & \multicolumn{2}{c}{CIFAR-100} \\
\cmidrule(lr{0.5em}){2-3}
\cmidrule(lr{0.5em}){4-5}
\multicolumn{1}{c}{}  & \begin{tabular}[c]{@{}c@{}}Params \\ (million)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Acc\\ (\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Params \\ (million)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Acc\\ (\%)\end{tabular} \\
\midrule
M1-50K&0.459&88.84&0.422&62.75\\
M2-50K&0.305&89.91&0.32&62.11\\
M3-50K&0.483&90.4&0.415&63.62\\
\midrule
M1-100K&1.83&91.49&1.66&69.07\\
M2-100K&1.217&92.18&1.26&68.67\\
M3-100K&0.856&91.57&0.734&67.52\\
\midrule
M1-500K&46.75&93.96&41.83&76.1\\
M2-500K&30.29&94.41&31.19&77.2\\
M3-500K&21.3&94.88&18.12&76.74\\
\midrule
M1-1M&189.2&94.34&169.1&78.13\\
M2-1M&124.14&95.00&127.7&79.07\\
M3-1M&89.46&95.37&76.01&78.73 \\
\bottomrule
\end{tabular}
\label{table:scale_budget}
\end{table}
%\end{wraptable}

==> tab_m3_relubudget_scaling.tex <==
%\begin{wraptable}{r}{0.7\textwidth}
\begin{table}
\caption{Comparison of scaled M3 to $50$K and $100$K ReLU budgets with equal ReLU an Equal FLOPs rules.
}
\begin{tabular}{lcccc}\toprule
\multicolumn{1}{c}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Model \\ (Base-Budget-Dataset)\end{tabular}}} & \multicolumn{2}{c}{R (Equal ReLUs)}& \multicolumn{2}{c}{E (Equal FLOPs)} \\
\cmidrule(lr{0.5em}){2-3}
\cmidrule(lr{0.5em}){4-5}
\multicolumn{1}{c}{} & \begin{tabular}[c]{@{}c@{}}Params \\ (million)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Acc\\ (\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Params \\ (million)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Acc\\ (\%)\end{tabular} \\
\midrule
M3-50K-C10&0.483&90.4&0.068&87.04\\
M3-100K-C10&0.856&91.57&0.208&90.58\\
\midrule
M3-50K-C100&0.415&63.62&0.062&44.83\\
M3-100K-C100&0.734&67.52&0.184&59.59 \\
\bottomrule
\end{tabular}
\label{table:scale_rule}
\end{table}
%\end{wraptable}

==> tab_orig_vs_shuffle_vs_prune.tex <==

\begin{table}[]
\caption{Comparing ReLU shuffling and ReLU pruning optimizations to original implimentationn on CIFAR-10/100. ReLU shuffling implements the same functionality as the original, and therefore doesn't affect accuracy.}
\begin{tabular}{lcccccccccc}\toprule
\multicolumn{1}{c}{\multirow{2}{*}{Model}} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Params \\ (million)\end{tabular}} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Original \\ Budget\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Shuffled \\ Budget\end{tabular}} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Orig Acc\\ (\%)\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Pruned\\ Budget\end{tabular}} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Pruned Acc\\ (\%)\end{tabular}} \\
\cmidrule(lr{0.5em}){2-3}
\cmidrule(lr{0.5em}){4-5}
\cmidrule(lr{0.5em}){7-8}
\cmidrule(lr{0.5em}){10-11}
\multicolumn{1}{c}{}
&C10&C100&C10&C100&&C10&C100&&C10&C100\\
\midrule
CNet1&0.459&0.422&147K&122K&100K&91.52&69.14&50K&88.84&62.75\\
CNet2&0.305&0.32&192K&192K&100K&90.71&66.46&50K&89.91&62.11\\
CNet3&0.483&0.415&411K&476K&100K&91.69&67.52&50K&90.4&63.62\\
\midrule
CNet1&1.83&1.66&295K&245K&200K&93.89&73.12&100K&91.49&69.07\\
CNet2&1.217&1.26&385K&385K&200K&93.08&72.77&100K&92.18&68.67\\
CNet3&0.856&0.734&548K&634K&200K&93.12&70.99&100K&91.57&67.52\\
\midrule
CNet1&46.75&41.83&1.49M&1.24M&1M&95.48&78.13&500K&93.96&76.1\\
CNet2&30.29&31.19&1.92M&1.92M&1M&95.47&79.71&500K&94.41&77.2\\
CNet3&21.3&18.12&2.74M&3.17M&1M&95.58&79.65&500K&94.88&76.74 \\
\bottomrule
\end{tabular}
\label{table:scale}
\end{table}

